MAXI and NuSTAR observations of the faint X-ray transient MAXI J1848-015 in the GLIMPSE-C01 Cluster

We present the results of MAXI monitoring and two NuSTAR observations of the recently discovered faint X-ray transient MAXI J1848-015. Analysis of the MAXI light-curve shows that the source underwent a rapid flux increase beginning on 2020 December 20, followed by a rapid decrease in flux after only $\sim5$ days. NuSTAR observations reveal that the source transitioned from a bright soft state with unabsorbed, bolometric ($0.1$-$100$ keV) flux $F=6.9 \pm 0.1 \times 10^{-10}\,\mathrm{erg\,cm^{-2}\,s^{-1}}$, to a low hard state with flux $F=2.85 \pm 0.04 \times 10^{-10}\,\mathrm{erg\,cm^{-2}\,s^{-1}}$. Given a distance of $3.3$ kpc, inferred via association of the source with the GLIMPSE-C01 cluster, these fluxes correspond to an Eddington fraction of order $10^{-3}$ for an accreting neutron star of mass $M=1.4M_\odot$, or even lower for a more massive accretor. However, the source spectra exhibit strong relativistic reflection features, indicating the presence of an accretion disk which extends close to the accretor, for which we measure a high spin, $a=0.967\pm0.013$. In addition to a change in flux and spectral shape, we find evidence for other changes between the soft and hard states, including moderate disk truncation with the inner disk radius increasing from $R_\mathrm{in}\approx3\,R_\mathrm{g}$ to $R_\mathrm{in}\approx8\,R_\mathrm{g}$, narrow Fe emission whose centroid decreases from $6.8\pm0.1$ keV to $6.3 \pm 0.1$ keV, and an increase in low-frequency ($10^{-3}$-$10^{-1}$ Hz) variability. Due to the high spin we conclude that the source is likely to be a black hole rather than a neutron star, and we discuss physical interpretations of the low apparent luminosity as well as the narrow Fe emission.

==> README <==
README for tablefootnote package, 2014/01/26, v1.1c


TABLE OF CONTENTS
=================

1 Introduction
2 Download
3 Installation
4 Additional Packages
5 Package Compatibility
6 Author/Maintainer
7 Bug Reports
8 Known Problems


1 INTRODUCTION
==============

This LaTeX package provides the command \tablefootnote{...}
to be used in a table or sidewaystable environment.
In those environments \footnote{...} would not work and
would need to be replaced by \footnotemark in the
(sideways)table and \footnotetext{...} after the
(sideways)table environment ended. Additionally the counters
for footnote and (when the hyperref package with option
hyperfootnotes=true is used) Hfootnote would need to be
adjusted manually. Then still the hyperlinks in a
(sideways)table would not work.
When the footnotebackref package is used, \footnotemark and
\footnotetext{...} would need to be redefined.
Just using \tablefootnote{...} in the (sideways)table does
all this automatically. (Compatibility with the
footnotebackref package was achieved without redefining
\footnotemark or \footnotetext.)
Redefining \footnote was not done as to not create conflicts
with other packages.
This material is subject to the LaTeX Project Public License
(LPPL). See http://www.ctan.org/license/lppl1.3
for the details of that license.


2 DOWNLOAD
==========

`tablefootnote' is available on CTAN:
  http://www.ctan.org/pkg/tablefootnote

Running
tex tablefootnote.dtx
generates the files
tablefootnote.ins, tablefootnote.drv, tablefootnote.sty,
and tablefootnote-example.tex.

Also a ZIP file is provided that contains these files,
the manual (tablefootnote.pdf), the compiled example
(tablefootnote-example.pdf), and this README, already
sorted in a TDS tree:
  http://www.ctan.org/install/macros/latex/contrib/
  tablefootnote.tds.zip

3 INSTALLATION
==============

Installation with ZIP file in TDS format
----------------------------------------
The ZIP file `tablefootnote.tds.zip' contains the files
sorted in a TDS tree. Thus you can directly unpack the
ZIP file inside a TDS tree.
(See CTAN:tds.zip for an explanation of TDS.)
Example:
  cd /...somewhere.../texmf
  unzip /...downloadpath.../tablefootnote.tds.zip
Do not forget to refresh the file name database of this
TDS tree.
Example:
  texhash /...somewhere.../texmf

Manual installation
-------------------
a) Download the tablefootnote files from CTAN.
   If necessary, unpack them.
b) Generate the package and driver files:
     tex tablefootnote.dtx
c) Install the file `*.sty' in your TDS tree:
     cp *.sty TDS:tex/latex/tablefootnote/
   Replace `TDS:' by the prefix of your TDS tree
   (texmf directory).
d) Create the documentation (if necessary), e.g.
     pdflatex  tablefootnote.dtx
     makeindex -s gind.ist  tablefootnote.idx
     pdflatex  tablefootnote.dtx
     makeindex -s gind.ist  tablefootnote.idx
     pdflatex  tablefootnote.dtx
e) Update the databases if necessary, e.g. for teTeX:
     mktexlsr .../texmf
f) Create the tablefootnote-example.pdf (if necessary), e.g.
     pdflatex tablefootnote-example.tex
     pdflatex tablefootnote-example.tex
     pdflatex tablefootnote-example.tex
g) Copy the documentation files to
   "TDS:doc/latex/tablefootnote/":
   README, tablefootnote.pdf, tablefootnote-example.tex,
   tablefootnote-example.pdf.


4 ADDITIONAL PACKAGES
=====================

tablefootnote loads other packages:
* letltxmacro, http://www.ctan.org/pkg/letltxmacro
* ltxcmds, http://www.ctan.org/pkg/ltxcmds
When the etoolbox package is available, it is used:
* etoolbox, http://www.ctan.org/pkg/etoolbox
(All packages possibly load further packages.
See the result of the \listfiles command in the log-file
of the example.)


5 PACKAGE COMPATIBILITY
=======================

- Using the hyperref-option pdfview=FitH or FitBH makes the
    hyperlinks of footnotes in sidewaystables to not lead
    to the footnotes, due to a bug in pdfTeX,
    computing wrong anchor coordinates (Heiko Oberdiek,
    29. October 2011). The printed version is OK.
- Footnotes in sidewaystables are printed one below the
    other, even if the footmisc package with option "para"
    is used.
- When LuaTeX is used to compile a document with
    rotated content, the hyperreferences therein are
    misplaced (regardless of loaded tablefootnote-package
    or footnotes at all - all hyperreferences in
    rotated content are misplaced). Using pdflatex does not
    result in any problem here.


6 AUTHOR/MAINTAINER
=====================

* H.-Martin Münch


7 BUG REPORTS
==============

A bug report should contain:
* Comprehensive problem description. This includes error or
  warning messages.
* \errorcontextlines=\maxdimen can be added in the
  TeX code to get more information in TeX error messages.
* Minimal test file that shows the problem, but does not
  contain any unnecessary packages and code.
* Used drivers/programs.
* Version information about used packages and programs.
* If you are using LaTeX, then add "\listfiles". Then
  a list of version information is printed at the end
  of the LaTeX run.
* Please no other files than the minimal test file.
  The other files .log, .dvi, .ps, .pdf are seldom
  necessary, so send them only on request.
* Please .zip or .tar.gz your file(s) before sending them!

Bug address
-----------
Bug reports can be send to the maintainer:
  H.-Martin Münch
  <Martin [dot] Muench [at] Uni-Bonn [dot] de>


8 KNOWN PROBLEMS
=================

- Using the hyperref-option "pdfview=FitH" or "pdfview=FitBH"
    makes the hyperlinks of footnotes in sidewaystables
    to not lead to the footnotes, due to a bug in pdfTeX,
    computing wrong anchor coordinates (Heiko Oberdiek,
    2011/10/29). The printed version is OK.
- Footnotes in sidewaystables are printed one below the other,
    even if the footmisc package with option para is used.
- When a table with (table)footnotes floates to another place,
    its footnotenumbers are not automatically adapted.
- When LuaTeX is used to compile a document with
    rotated content, the hyperreferences therein are
    misplaced (regardless of loaded tablefootnote-package
    or footnotes at all - all hyperreferences in
    rotated content are misplaced). 
    Using pdflatex does not result in any problem here.
    Problem found by Arno Trautmann, 2011/11/15.

Ideas for solutions are welcome!
